Clever Hans or Neural Theory of Mind? Stress Testing Social Reasoning in Large Language Models

The escalating debate on AI's capabilities warrants developing reliable metrics to assess machine "intelligence". Recently, many anecdotal examples were used to suggest that newer large language models (LLMs) like ChatGPT and GPT-4 exhibit Neural Theory-of-Mind (N-ToM); however, prior work reached conflicting conclusions regarding those abilities. We investigate the extent of LLMs' N-ToM through an extensive evaluation on 6 tasks and find that while LLMs exhibit certain N-ToM abilities, this behavior is far from being robust. We further examine the factors impacting performance on N-ToM tasks and discover that LLMs struggle with adversarial examples, indicating reliance on shallow heuristics rather than robust ToM abilities. We caution against drawing conclusions from anecdotal examples, limited benchmark testing, and using human-designed psychological tests to evaluate models.

==> Tables/tomi_tomk_comparison.tex <==
\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}c|cc|c@{}}
\toprule
\textbf{Dataset} & \multicolumn{2}{c|}{\textbf{ToMi'}} & \textbf{ToM-k} \\ \midrule
\textbf{Setup}                                                      
& \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Zero-shot\\ all question\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}c@{}}Zero-shot\\ w.o second order\\ questions\end{tabular}} & \textbf{Zero-shot}  \\ \midrule
\textbf{\begin{tabular}[c]{@{}c@{}}GPT 3.5 \\ Accuracy\end{tabular}} %& \multicolumn{1}{c|}{42.5} 
& \multicolumn{1}{c|}{0.10}                                                                      & 0.21                                                                                      & 0.87        \\   \bottomrule    
\end{tabular}%
}
\caption{Sally-Anne false belief tests comparison between ToM-k, that contains positive examples only and ToMi', that contain both positive and negative examples (manually adjusted from ToMi to be of the same probing type as ToM-k). ToM-k contains only first-order questions. The subset ``Zero-shot w.o second-order questions'' was created manually to better compare to ToM-k dataset. Lower scores indicates stronger dataset.}
\label{tab:tomi_tomk_comparison_old}
\end{table}
